Fair Sequential Selection Using Supervised Learning Models

We consider a selection problem where sequentially arrived applicants apply for a limited number of positions/jobs. At each time step, a decision maker accepts or rejects the given applicant using a pre-trained supervised learning model until all the vacant positions are filled. In this paper, we discuss whether the fairness notions (e.g., equal opportunity, statistical parity, etc.) that are commonly used in classification problems are suitable for the sequential selection problems. In particular, we show that even with a pre-trained model that satisfies the common fairness notions, the selection outcomes may still be biased against certain demographic groups. This observation implies that the fairness notions used in classification problems are not suitable for a selection problem where the applicants compete for a limited number of positions. We introduce a new fairness notion, ``Equal Selection (ES),'' suitable for sequential selection problems and propose a post-processing approach to satisfy the ES fairness notion. We also consider a setting where the applicants have privacy concerns, and the decision maker only has access to the noisy version of sensitive attributes. In this setting, we can show that the perfect ES fairness can still be attained under certain conditions.

==> Preliminary.tex <==
\section{Preliminary}

\subsection{Privacy preserving selection algorithm}
Let $x_i\in \mathcal{X}$ be the realization of individual $i$'s feature vector, %be a vector with dimension $d$ denoting the data of individual $i$, 
and $D=(x_1, x_2,\ldots, x_n)$ be a dataset of all individuals' data, and $\mathcal{D} = \{(\hat{x}_1,\hat{x}_2,\ldots,\hat{x}_n)| \hat{x}_i \in \mathcal{X} \}$ denotes the set of all possible datasets. 

\begin{definition}[Neighboring Datasets]
	%We say 
	Two datasets $D = (x_1,\ldots, x_n)$ and $D' = (x'_1,\ldots, x'_n)$ are neighboring datasets if they differ only in one data point.That is, $\linebreak
	\exists i \in \mathcal{N} \mbox{ s.t. } x_i\neq x'_i~ \mbox{and} ~ x_j=x'_j~ \forall j \neq i.
	$. For notational convenience, $D\sim D'$ denotes that $D$ and $D'$ are neighboring data sets. 
\end{definition} 

\begin{definition}[The Laplace Distribution]
	A random variable has a Laplace distribution if its probability density function is equal to $g(x) = \frac{1}{2b} \exp\{-\frac{|x|}{b}\}$, where $b$ is the parameter of the Laplace distribution. For notational convenience, $Lap(b)$ denotes a random variable with the Laplace distribution and parameter $b$. 
\end{definition}
In this work, we use the notion of differential privacy to measure the privacy guarantee of the selection algorithm. 
%Consider randomized algorithm $M:\mathbb{D}\rightarrow \mathbb{R}$. If algorithm $M(.)$ is differentially private, the distribution of its output  should remain almost the same for two neighboring  databases. Differential privacy is mathematically defined as follows.  

\begin{definition}[Differential Privacy \cite{dwork2006differential}]
	A randomized algorithm $\mathscr{M}$ is 
	$\epsilon$-differentially private if for any two neighboring datasets $D$ and $D'$ and for any possible set of output $\mathcal{W}\subseteq \text{Range}(\mathscr{M})$, it holds that
	$
	\frac{{\Pr}\{\mathscr{M}(D)\in \mathcal{W}\}}{{\Pr}\{\mathscr{M}(D')\in \mathcal{W}\}} \leq \exp\{\epsilon\}.
	$
\end{definition}
Privacy parameter $\epsilon\in [0,\infty)$ provides a measure of the privacy guarantee; a smaller $\epsilon$ implies a stronger privacy guarantee. For sufficiently small $\epsilon$, an adversary is not able to identify the input data with high confidence because the distribution of  output remains almost the same regardless of changing one data point. %Next we introduce %It suggests that an attacker cannot infer the input data with high confidence after observing the output; thus, individual privacy is preserved. 
Next, we introduce a notable 
mechanism that can achieve differential privacy.% to generate differentially private outputs.  
\begin{definition}[Above Threshold Algorithm (\cite{TCS042}, Section 3.6) ]
	Let $f_i:\mathcal{D}\to \mathbb{R},i=1,2,\ldots $ be a sequence of query  functions. Assume that the sensitivity of each query function $f_i(\cdot)$ is 1. That is, $\max_{D\sim D'} |f_i(D)-f_i(D')| = 1, i=1, 2,. \ldots$. Assume that our task is to observe a sequence of queries $f_1(D), f_2(D), \dots $ and compare them with a public threshold $\tau$ and stop whenever a query above threshold $\tau$ is found. The algorithm \ref{alg:Above} (called Above Threshold)  is an $\epsilon$-differentially private algorithm which releases a bit vector indicating whether $f_i(D)$ is above threshold $\tau$ or not. 
	\begin{algorithm}
		\caption{Above Threshold}
		\label{alg:Above}
		\begin{algorithmic}
			\STATE {\bfseries Input:} data set $D$, $f_1, f_2, \ldots$, privacy parameter $\epsilon$
			\STATE $T = \tau + Lap(\frac{2}{\epsilon})$
			\FOR{Each query $i$}
			\STATE $V_i = Lap(\frac{4}{\epsilon})$
			\IF{$f_i(D)+V_i \geq T$}
			\STATE release $a_i=1$
			\STATE Halt.
			\ELSE
			\STATE release $a_i=0$	
			\ENDIF
			\ENDFOR
		\end{algorithmic}
	\end{algorithm}
\end{definition}
\vspace{-0.75cm}

==> Privacy.tex <==
\section{Selection with a Privacy Guarantee}
In order to preserve applicants' privacy, we use the Above Threshold algorithm. 
